StressNet: Detecting Stress in Thermal Videos

Precise measurement of physiological signals is critical for the effective monitoring of human vital signs. Recent developments in computer vision have demonstrated that signals such as pulse rate and respiration rate can be extracted from digital video of humans, increasing the possibility of contact-less monitoring. This paper presents a novel approach to obtaining physiological signals and classifying stress states from thermal video. The proposed network--"StressNet"--features a hybrid emission representation model that models the direct emission and absorption of heat by the skin and underlying blood vessels. This results in an information-rich feature representation of the face, which is used by spatio-temporal network for reconstructing the ISTI ( Initial Systolic Time Interval: a measure of change in cardiac sympathetic activity that is considered to be a quantitative index of stress in humans ). The reconstructed ISTI signal is fed into a stress-detection model to detect and classify the individual's stress state ( i.e. stress or no stress ). A detailed evaluation demonstrates that StressNet achieves estimated the ISTI signal with 95% accuracy and detect stress with average precision of 0.842. The source code is available on Github.

==> NO2_introold.tex <==
\section{Introduction}\label{sec:intro}

As the world has come to a standstill situation due to a deadly pandemic~\cite{roser2020coronavirus}, the need for non-contact physiological signal measurement based health systems are needed now more than ever. In this aspect, many of the recent researches in the area of remote  photoplethysmography (rPPG) ~\cite{wang2016algorithmic} have put focus on leveraging modern computer vision based systems ~\cite{chen2018deepphys,yu2019remote,mcduff2014remote,bousefsaf2013remote} to monitor human vitals such as heart rate and breathing rate. More recent works have expanded to detecting more complex human vitals such as stress levels ~\cite{yu2019remote,mcduff2014remote,bousefsaf2013remote}.
    

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{diagrams/ecg_icg.png}
\end{center}
   \caption{ ECG and ICG signals are plotted against time. After each ECG peak value there exists an ICG peak value. Time difference between these two values are known as PEP.         %\vspace{-0.5cm}
   }
\label{fig:ecg-icg}
\end{figure} 

    Interestingly none of the existing methods have utilized the strong physiological signals like pre-ejection time period (PEP) or initial systolic time interval (ISTI) to measure or quantify stress. PEP basically measures the time difference between the start of the electrical depolarization of left ventricle and the beginning of left ventricular ejection ~\cite{lanfranchi2010cardiovascular,blechert2016anslab}. Quantitatively, PEP can be obtained by simultaneous recording of the thoracic impedance cardiogram (ICG) and electrocardiogram (ECG) and is defined as the interval from the onset of left ventricular depolarization, reflected by the Q-wave onset in the ECG, to the opening of the aortic valve, reflected by the B-point in the ICG signal ~\cite{willemsen1996ambulatory, riese2003large}. Figure \ref{fig:ecg-icg} displays the ECG and ICG signals with the relevant landmarks. PEP is considered as a vital index of myocardial contractility ~\cite{newlin1979pre} and numerous efforts have shown that PEP can be used as a strong cue to analyze different physiological phenomena e.g. stress, blood pressure ~\cite{kelsey2012beta, prasad2017detection,forouzanfar2019automatic,hinnant2011developmental,brenner2011pre}. Other physiological signals cannot measure the changes in contractility which are influenced by sympathetic but not parasympathetic activity in humans ~\cite{newlin1979pre}.
    \begin{figure*}[t]
\begin{center}
\includegraphics[width=\linewidth,height=5cm]{diagrams/model_architecture.png}
\end{center}
   \caption{Model Architecture. Green boxes are the different modules of the model. Yellow  boxes are the variables throughout the model. Emission model process the raw input data which is then fed into spatial and temporal module. Detector network predicts PEP value for each of the frame from the output of these modules. This PEP signal is used as input in our stress detection network.  
  % \vspace{-0.5cm}
   }
\label{fig:model_architecture}
\end{figure*} 

    StressNet has leveraged this powerful PEP signal to detect if a person is under stress or not. For estimating the PEP signal a spatial-temporal neural network has been developed. In recent times there are many deep learning based works on detecting heart rate or heart rate variability ~\cite{yu2019remote,chen2018deepphys, hsu2017deep,niu2018synrhythm}. Most of these methods either fail to correctly use the peak information of the heart rate or did not properly use temporal relations in the face videos ~\cite{yu2019remote}. A very recent work by ~\cite{yu2019remote} has developed a spatial-temporal deep network to measure rPPG signals such as heart rate variability (HRV), average heart rate (AHR). Although these measurements are important, we argue that PEP signals are better indicator on estimating physiological phenomenon like stress. Our extensive experimental results have shown that   
    PEP acts as a strong prior while detecting stress. To the best of our knowledge StressNet is the first non-contact based approach to estimate the complicated PEP signal. Also, most of the deep learning methods like ~\cite{yu2019remote, chen2018deepphys} used RGB videos to estimate physiological signals. Although collecting or analyzing RGB videos are very much convenient these days, RGB videos suffer from lighting issues which can adversely effect the estimation of PEP signals or HRV. To circumvent this lighting issue StressNet has used thermal videos to estimate PEP signals. 
    
    In summary, StressNet is an end to end spatial temporal network that estimates PEP signal from the thermal videos of the face. An extensive analysis on the detailed dataset developed for this work has shown higher co-relation between the estimated signal and the ground truth. Also, the effectiveness of this predicted PEP signal is validated by detecting physically induced stress in thermal videos. 
    
    \vspace{0.3cm}
    \textbf{Technical Contributions:}
 \begin{itemize}
  \item We propose a spatial temporal deep neural network to estimate PEP signal. To the best of our knowledge this is the first attempt to directly estimate PEP signal from videos.
  \item With the extensive analysis on we have shown how this estimated PEP signal can be used to detect physiological phenomenon like stress.  
\end{itemize}

%\subsection{Related Work}

%\subsection{Proposed Method}

%\subsection{Technical Contributions}

%\subsection{Dataset}

==> Tom_Addition_Notes.tex <==
R1C2: Issue with faces going out of Frame.

%LIMITATIONS: The data were collected as part of a much larger project.  Participants were positioned in a chin-rest and a static thermal camera was trained on the face, which should have mitigated the need for a thermal image tracker.  However, despite our best efforts and clear instructions, participants did occasionally move their face from the chin rest, such as when they were transferring their feet too and from the water bucket, hence the issues.


R1C3: Issue with warm-water control.

%METHODS: The control task (WPT) was designed to be as similar in nature to the CPT, such that participants engaged in exactly the same protocol but without the discomfort associated with immersing the feet in ice water.  This was important, as it ensured that any psychological or physiological effects induced by the protocol or by water immersion per-se, were controlled for. [TOM PROVIDE CITATIONS SUPPORTING THE USE OF THE CPT + REF OUR PREPRINT?]

%LIMITATIONS: It is possible that the lukewarm-water immersion in the control condition, which was intended to induce a neutral state, may have actually induced a relaxed, positive state. [POSSIBLY REF OUR MANUSCRIPT TO SHOW THIS WASN'T THE CASE?]  


R1C3: Issue with subjects' waiting 25 mins between dips. Could this induce stress?  How do we keep them sane between dips?

%METHODS: In between CPT/WPT exposures, participants engaged in cognitive tasks designed to test performance across a range of cognitive domains.  The main goal of the study was to test stress effects on cognitive performance.  *I need to reframe the first few paragraphs of the methods section to clarify that the key goal of the BOSS study was to measure stress effects on brain, behavior, physio.

%LIMITATIONS: Data collection protocol was not specifically designed for the purposes of this analysis, so it is possible that participants completing the cognitive tasks in between CPT/WPT exposures may have impacted the outcomes etc.  But, consistent across conditons. 


R1C3: Data collection failures

%METHODS: XX participants' data were excluded due to technical failures (the thermal imaging camera failed to record one or more sessions).


%R1C3: No consent statement

%METHODS: Informed consent was obtained before the start of each experiment, and all procedures were approved by the BLAH (WIRB, US Army - see Alex Manuscript?)


R3C4: Dataset was collected in an extremely compact environment, so perhaps not realistic to "real world" scenarios where more atmospheric noise etc.

%LIMITATIONS: The data were collected under laboratory conditions and it is possible that noise, movement etc. might impact the accuracy of the model.  This will be explored in follow-up work...


%R3C4: Comment on high quality ICG data.  

%Not relevant - ignore


%R3C4: Comment on stress/HR.

%Not sure how to interpret this?  Ignore?


%R3C4: The term "stress" encompasses a wide range of states.  Suggests applying model to data collected under different stress scenarios to see how this ISTI metric applies.

%LIMITATIONS: The present paper only tests model performance under one specific type of stress: exposure to a noxious stimulus.  As such, it is unclear whether the model can also discriminate other forms of stress e.g. social stress, fatigue etc.  Future work...


R3C4: Lack of comparison between non-contact ISTI method and other contact methods of stress detection.

%I think just ignore this because it's beyond scope of manuscript.  Or, we add a sentence stating that follow-up work will do this.  I'm tempted to just ignore.


R4C3: PEP over-explanation

I agree with the reviewer - cut this down/out!


R4C3: Privacy concerns even with thermal cameras

Yeah, I kinda agree.  You can still make out the person with the thermal camera so claiming anonymity is a bit of a stretch.  Perhaps something could be applied as part of the recording to conceal the face identity?  Do we even need to record at all?


R4C4: Figure captions require more explanation.

Tom look at these and make suggestions later.


%R4C4: lack of clarity about why some subjects were removed, and how many.

%Tom edit for clarity.  Explain why subs were rejected (technical issues - see earlier reviewer's point as well)

%R4C4: rename StressNet to ISTInet

%Probably ignore






% NOTES
% Ask PIs about 1) Preprint 2) Data available online?


